Improving Generalization of Adversarial Training via Robust Critical Fine-Tuning

Deep neural networks are susceptible to adversarial examples, posing a significant security risk in critical applications. Adversarial Training (AT) is a well-established technique to enhance adversarial robustness, but it often comes at the cost of decreased generalization ability. This paper proposes Robustness Critical Fine-Tuning (RiFT), a novel approach to enhance generalization without compromising adversarial robustness. The core idea of RiFT is to exploit the redundant capacity for robustness by fine-tuning the adversarially trained model on its non-robust-critical module. To do so, we introduce module robust criticality (MRC), a measure that evaluates the significance of a given module to model robustness under worst-case weight perturbations. Using this measure, we identify the module with the lowest MRC value as the non-robust-critical module and fine-tune its weights to obtain fine-tuned weights. Subsequently, we linearly interpolate between the adversarially trained weights and fine-tuned weights to derive the optimal fine-tuned model weights. We demonstrate the efficacy of RiFT on ResNet18, ResNet34, and WideResNet34-10 models trained on CIFAR10, CIFAR100, and Tiny-ImageNet datasets. Our experiments show that \method can significantly improve both generalization and out-of-distribution robustness by around 1.5% while maintaining or even slightly enhancing adversarial robustness. Code is available at https://github.com/microsoft/robustlearn.

==> tables/tb-ablation-different-module.tex <==
% \begin{table}[t!]

% \caption{Results of fine-tuning on different modules. All methods help improve the generalization and OOD robustness, but only fine-tuning on non-robust critical module can alleviate the trade-off between adversarial robustness and generalization.}
% \label{table: fine-tuning on different modules}
% \centering
% %\begin{center}
% \begin{tabular}{ c c c c}

% \toprule

% Method & Std & OOD & Adv \\


% \midrule
% Base & 81.46 & 73.56 & 53.63 \\
% All layers & 83.56 & 75.48 & 52.66 \\
% Last layer & 83.35 & 75.16 & 52.75 \\
% Robust Critical & 83.36 & 75.42 & \color{Green} 52.48 \\
% Non-robust Critical & 83.44 & 75.69 & \textbf{53.65} \\
% \bottomrule
% \end{tabular}
% %\end{center}

% \end{table}

==> tables/tb-ablation-more-non-critical-modules.tex <==
% \begin{table}[t!]

% \caption{Fine-tuning on multiple non-robust critical modules.}
% \label{table: fine-tuning on multiple modules}
% \centering
% %\begin{center}
% \begin{tabular}{ c c c c}

% \toprule

% Method & Std & OOD & Adv \\
% \midrule
% Top1 & 83.44 & & \textbf{53.65} \\
% Top2 & 83.41 & & 52.47 \\
% Top3 & 83.59 & & 52.22 \\
% Top5 & 83.70 & & 52.35 \\
% \bottomrule
% \end{tabular}
% %\end{center}

% \end{table}


